SAMIC: Segment Anything with In-Context Spatial Prompt Engineering

Few-shot segmentation is the problem of learning to identify specific types of objects (e.g., airplanes) in images from a small set of labeled reference images. The current state of the art is driven by resource-intensive construction of models for every new domain-specific application. Such models must be trained on enormous labeled datasets of unrelated objects (e.g., cars, trains, animals) so that their ``knowledge'' can be transferred to new types of objects. In this paper, we show how to leverage existing vision foundation models (VFMs) to reduce the incremental cost of creating few-shot segmentation models for new domains. Specifically, we introduce SAMIC, a small network that learns how to prompt VFMs in order to segment new types of objects in domain-specific applications. SAMIC enables any task to be approached as a few-shot learning problem. At 2.6 million parameters, it is 94% smaller than the leading models (e.g., having ResNet 101 backbone with 45+ million parameters). Even using 1/5th of the training data provided by one-shot benchmarks, SAMIC is competitive with, or sets the state of the art, on a variety of few-shot and semantic segmentation datasets including COCO-$20^i$, Pascal-$5^i$, PerSeg, FSS-1000, and NWPU VHR-10.

==> app_embedding.tex <==
\begin{figure}[htpb]
    \centering
    \includegraphics[width=\linewidth]{figures/persam_problems3.pdf}
    \caption{\textbf{Illustration of key limitations of training-free,  embedding similarity-based spatial prompt engineering methods.} %These methods typically (a) struggle with visual distractions, (b) generalize poorly, (c) cannot handle multiple visual object instances and (d) perform poorly on domain-specific tasks. Here, PerSAM \cite{zhang2023personalize} is used as a test bed for performing empirical observations. Sample target images of where PerSAM fails in each category are shown.
    }
    \label{fig:persam_problems}
\end{figure} 



To further examine the limitations of similarity-based methods, we conduct extensive empirical experiments using PerSAM \cite{zhang2023personalize} as the test bed, as shown in \cref{fig:persam_problems}. PerSAM generates positive (\textcolor{RoyalBlue}{\ding{72}}) and negative (\textcolor{red}{\ding{72}}) point prompts based on an in-context sample consisting of an image and its mask. Our experiments reveal the following key issues: (i) \emph{Susceptibility to visual distractions}—demonstrated in \cref{fig:persam_problems}(a), where correspondence maps may highlight unrelated objects sharing similar features, and positive prompts are often biased toward the image center. (ii) \emph{Poor generalization}—as shown in \cref{fig:persam_problems}(b), where objects with different visual features fail to be detected despite belonging to the same category. (iii) \emph{Inability to handle multiple instances}—highlighted in \cref{fig:persam_problems}(c), where only one instance is typically identified when multiple are present. (iv) \emph{Suboptimal performance on domain-specific tasks}—such as medical or remote sensing segmentation (\cref{fig:persam_problems}(d)). This occurs because (1) generic pre-trained VFMs lack training on domain-specific data, leading to inadequate embeddings, and (2) a single pair of positive-negative prompts results in ambiguous segmentation, as noted in the SAM paper \cite{kirillov2023segment}. 

